Theoretical possibilities for flat-band superconductivity

One novel arena for designing superconductors with high $T_C$ is the flat-band systems. A basic idea is that flat bands, arising from quantum mechanical interference, give unique opportunities for enhancing $T_C$ with (i) many pair-scattering channels between the dispersive and flat bands, and (ii) an even more interesting situation when the flat band is topological and highly entangled. Here we compare two routes, which comprise a multi-band system with a flat band coexisting with dispersive ones, and a one-band case with a portion of the band being flat. Superconductivity can be induced in both cases when the flat band or portion is "incipient" (close to, but away from, the Fermi energy). Differences are, for the multi-band case, we can exploit large entanglement associated with topological states, while for the one-band case a transition between different (d and p) wave pairings can arise. These hint at some future directions.

==> bibitem.tex <==
\begin{thebibliography}{}
%
% and use \bibitem to create references. Consult the Instructions
% for authors for reference list style.

\bibitem{sakakibara} H. Sakakibara et al., Phys. Rev. Lett. {\bf 105}, 057003 (2010); Phys. Rev. B {\bf 85}, 064501 (2012); {\bf 86}, 134520 (2012); {\bf 89}, 224505 (2014).


\bibitem{kobayashi} K. Kobayashi, M. Okumura, S. Yamada, M. Machida, and H. Aoki, Phys. Rev. B {\bf 94}, 214501 (2016).


\bibitem{sayyad} S. Sayyad, E. W. Huang, M. Kitatani, M.-S. Vaezi, Z. Nussinov, A. Vaezi and H. Aoki, Phys. Rev. B {\bf 101}, 014501 (2020).

\bibitem{narrowwide} K. Kuroki, T. Higashida, and R. Arita, Phys. Rev. B {\bf 72}, 212509 (2005).


\bibitem{kobayashi_added} K. Kobayashi, M. Okumura, S. Yamada, M. Machida, and H. Aoki, unpublished.



\bibitem{noack94} R.M. Noack, S.R. White and D.J.Scalapino, Phys. Rev. Lett. {\bf 73}, 882 (1994).  In the Tomonaga-Luttinger theory, 
a pairing is called d-wave-like when the 
pair wave function has opposite signs between 
the bonding and antibonding bands, as in 
L. Balents and M.P.A. Fisher, Phys. Rev. B {\bf 53}, 12133 (1996). 


\bibitem{kuroki96} K. Kuroki, T. Kimura and H. Aoki, Phys. Rev. B {\bf 54}, R15641 (1996).


\bibitem{matsumoto} K. Matsumoto, D. Ogura, and K. Kuroki, Phys. Rev. B {\bf 97}, 014516 (2018).  

\bibitem{misumi} T. Misumi and H. Aoki, Phys. Rev. B {\bf 96}, 155137 (2017).

\bibitem{azurite} H. Kikuchi et al., Phys. Rev. Lett. {\bf 94}, 227201 (2005); H. Jeschke et al., Phys. Rev. Lett. {\bf 106}, 217201 (2011).

\bibitem{ogura} D. Ogura, H. Aoki and K. Kuroki, Phys. Rev. B {\bf 96}, 184513 (2017).


\bibitem{vaezi} E. W. Huang, M.-S. Vaezi, Z. Nussinov, and A. Vaezi, Phys. Rev. B {\bf 99}, 235128 (2019).

\bibitem{kitatani} M. Kitatani, N. Tsuji and H. Aoki, Phys. Rev. B  {\bf 92}, 085104 (2015).

\bibitem{hosonoKuroki} H. Hosono and K. Kuroki, Physica C {\bf 514}, 399 (2015).

\bibitem{arita} P. Monthoux and G. G. Lonzarich, Phys. Rev. B {\bf 59}, 14598 (1999); R. Arita, K. Kuroki, and H. Aoki, Phys. Rev. B {\bf 60}, 14585 (1999).

\bibitem{kitataniDGA} M. Kitatani, T. Sch\"{a}fer, H. Aoki and K. Held, Phys. Rev. B {\bf 99}, 041115(R) (2019).

\bibitem{murakami} Y. Murakami, T. Oka and H. Aoki, Phys. Rev. B {\bf 88}, 224404 (2013).

\bibitem{torma} S. Peotta and P. T\"{o}rm\"{a}, Nature Commun. {\bf 6}, 8944 
(2015); M. Tovmasyan et al., Phys. Rev. B {\bf 94}, 245149 (2016); {\bf 98}, 134513 (2018).

\bibitem{liu2018} C. C. Liu et al., Phys. Rev. Lett. {\bf 121}, 217001 (2018).

\bibitem{fernandes2013} F. M. Fernandes and A. J. Millis, Phys. Rev. Lett. 
{\bf 111}, 127001 (2013); F. Ahn et al., Phys. Rev. B {\bf 89}, 144513 (2014).

\bibitem{TBG} Y. Cao, V. Fatemi, S. Fang, K. Watanabe, T. Taniguchi, E. Kaxiras, and P. Jarillo-Herrero, Nature {\bf 556}, 43 (2018); 
X. Lu et al, Nature {\bf 574}, 653 (2019).

\bibitem{Guinea} F. Guinea and N.R. Walet, Proc. Nat. Acad. Sci. {\bf 115}, 
13174 (2018).

\bibitem{Vishwanath} H.C. Po et al, Phys. Rev. B {\bf 99}, 195455 (2019).

\bibitem{akashi} R. Akashi, arXiv:1909.02956.

\bibitem{kurokiQMC} K. Kuroki and H. Aoki, Phys. Rev. B {\bf 42}, 2125 (1990); Phys. Rev. Lett. {\bf 69}, 3820 (1992); Phys. Rev. B {\bf 48}, 7598 (1993).

\bibitem{kurokiBosonisation} K. Kuroki and H. Aoki, 
Phys. Rev. Lett. {\bf 72}, 2947 (1994).

\bibitem{agrestini} S. Agrestini et al, J. Phys. A {\bf 36}, 9133 (2003). 

\bibitem{tajima} H. Tajima et al, Physical Review B {\bf 99}, 180503 (2019).

\bibitem{bussmann} A. Bussmann-Holder et al, Condensed Matter {\bf 2}, 24 (2017).

\bibitem{kagan} M.Y. Kagan and A. Bianconi, Condensed Matter {\bf 4}, 51 (2019).
\bibitem{bianconiJarlborg}  A. Bianconi and T. Jarlborg, Europhysics Letters {\bf 112}, 37001 (2015). 

\end{thebibliography}

% end of file template.tex


